A Bayesian analysis of the time through the order penalty in baseball

As a baseball game progresses, batters appear to perform better the more times they face a particular pitcher. The apparent drop-off in pitcher performance from one time through the order to the next, known as the Time Through the Order Penalty (TTOP), is often attributed to within-game batter learning. Although the TTOP has largely been accepted within baseball and influences many managers' in-game decision making, we argue that existing approaches of estimating the size of the TTOP cannot disentangle continuous evolution in pitcher performance over the course of the game from discontinuities between successive times through the order. Using a Bayesian multinomial regression model, we find that, after adjusting for confounders like batter and pitcher quality, handedness, and home field advantage, there is little evidence of strong discontinuity in pitcher performance between times through the order. Our analysis suggests that the start of the third time through the order should not be viewed as a special cutoff point in deciding whether to pull a starting pitcher.

==> model_simulations.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model simulation study}\label{sec:model_sim}

We conduct a simulation study to assess the capacity of our model (Equation~\eqref{eqn:model}) to estimate time through the order penalties of various sizes.
Specifically, we simulate data consistent with different $\ttops$ and verify that our posterior estimates are close to the data generating parameters. 

\textbf{Simulation setup.}
For our first simulation, we generate data consistent with continuous pitcher fatigue and no $\ttop$ for any of the plate appearance outcomes by setting $\beta_{2k} = \beta_{3k} = 0$ for each $k \neq 1.$
In our second simulation, for each $k \neq 1,$ we set the $\beta_{2k}$ and $\beta_{3k}$ so that the resulting $\xwoba$ curves display $\ttops$ consistent with \citet{theBook}'s findings of about 10 expected $\woba$ points between successive times through the order.
%the alleged effect size from \citet{theBook} of about 10 $\woba$ points between each time through the order.
Finally, for our third simulation, we set $\beta_{2k}$ and $\beta_{3k}$ so that there is no $\ttoptwo$ (in terms of $\xwoba$) but a large $\ttopthree$ of about 50 $\woba$ points. 
For each simulation, we set the values of the $\alpha_{0k}$'s, $\alpha_{1k}$'s, and $\eta_{k}$'s in a way that is consistent with observed data. 
Additional details about the simulation setup, including the data generating parameter values, are available in Appendix~\ref{app:simulation_details}.

For each simulation, we generate 25 full seasons worth of data.
We fit our model to 80\% of the data from each simulated season and evaluate our fitted model's predictive performance on the remaining 20\%.
We further assess how well our fitted model recovers the function $\xwoba(t,\bx)$ for a set of average confounder values. 
% In particular, \skd{explain this bit further}

%We then gather our observed data $\{t_i\}$ and $\{X_{i\ast}\}$ from 2018, consisting of every plate appearance in 2018. 
%Then, for each of our three simulation studies, we use our ``true'' simulation parameters to generate 25 independent draws of $y$ according to Model~\ref{eqn:model}. Then, we split these 25 simulated datasets into 25 training and testing sets, where the training set consists of a random 80\% of the full set. Using these 25 training datasets, we estimate the posterior distribution of our parameters, from Formula~\ref{eqn:posterior_dist}, yielding 25 posterior distributions $\{(\alpha^{(j)}, \beta^{(j)}, \eta^{(j)})\}_{j=1}^{25}$. Using these 25 testing sets, we evaluate the performance of Model~\ref{eqn:model} by computing several metrics with these posterior distributions, detailed in Section~\ref{sec:simResults}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\textbf{Simulation results.}
In all three simulation studies, we reliably recover the data generating parameters: averaged across all parameters, the estimated frequentist coverage of the marginal 95\% posterior credible intervals exceeds 88\% in each study. 
Importantly, the coverage of the 95\% posterior credible intervals for the discontinuity parameters $\beta_{2k}$ and $\beta_{3k}$ is 100\%.
That is, for each simulated dataset, the 95\% credible intervals for the $\beta_{2k}$'s and $\beta_{3k}$'s always contain the true data generating parameters.
Furthermore, our model demonstrates good predictive capabilities (see Appendix~\ref{app:simulation_details} for details).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Simulation visualization.}
In each simulation, we visualize the trajectory of posterior expected $\woba$ over the course of the game for an average batter on the road facing an average pitcher with the same handedness.
That is, we plot the sequence $\{\xwoba(t,\tilde{\bx})\}_{t = 1}^{27}$ where 
\begin{equation}
\label{eqn:x_tilde}
\tilde{\bx}^\top = (\text{logit}(0.315), \text{logit}(0.315), 1, 0).
\end{equation}
Figure~\ref{fig:plotXwobaSims} shows the sequence of posterior means, 50\%, and 95\% credible intervals of $\xwoba(t,\tilde{\bx})$ based on a single simulated dataset from each simulation setting.
We overlay the true values of $\xwoba(t,\tilde{\bx}),$ computed from the data generating parameters, to each plot. 
We see that in each of the three simulation studies, we recover the true underlying expected $\woba$  trajectory. 
Although there is some bias in the second simulation, the magnitude of the bias is small, and the true expected $\woba$  values lie in the 50\% credible intervals.


%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{plots/plot_sim1_s1_xwoba_check_post_paper}
% \caption{}
\label{fig:XwobaSim1}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{plots/plot_sim2_s1_xwoba_check_post_paper}
% \caption{}
\label{fig:XwobaSim2}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{plots/plot_sim3_s6_xwoba_check_post_paper}
% \caption{}
\label{fig:XwobaSim3}
\end{subfigure}
    \caption{Trend in $\xwoba$ over the course of a game from our first, second, and third simulation studies.
    The red dots indicate the true underlying expected $\woba$ values, the white dots indicate the posterior means of the $\xwoba$ values, the thick black error bars denote the 50\% posterior credible intervals, and the thin black error bars denote the 95\% posterior credible intervals.}
    \label{fig:plotXwobaSims}%
\end{figure}





% \begin{figure}[H]
% \centering
% \includegraphics[width=10cm]{plots/plot_sim1_s1_xwoba_check_post.png}
% \caption{Trend in expected wOBA (from Formula~\ref{eqn:xwoba_seq}) over the course of a game from our first simulation study, in which there is pitcher fatigue but no TTOP. The red dots indicate the ``true'' underlying expected wOBA trajectory, the white dots indicate the posterior means of the expected wOBA values, the thick black error bars denote the 50\% credible intervals, and the thin black error bars denote the 95\% credible intervals. We succesfully recover the ``true'' underlying expected wOBA function.} 
% \label{fig:plotXwobaSim1}
% \end{figure}

% \begin{figure}[H]
% \centering
% \includegraphics[width=10cm]{plots/plot_sim2_s1_xwoba_check_post.png}
% \caption{Trend in expected wOBA (from Formula~\ref{eqn:xwoba_seq}) over the course of a game from our second simulation study, in which there is pitcher fatigue and a 2TTOP and a 3TTOP consistent with Tom Tango's alleged effect size of about 10 wOBA points from one TTO to the next. The red dots indicate the ``true'' underlying expected wOBA trajectory, the white dots indicate the posterior means of the expected wOBA values, the thick black error bars denote the 50\% credible intervals, and the thin black error bars denote the 95\% credible intervals. We succesfully recover the ``true'' underlying expected wOBA function.} 
% \label{fig:plotXwobaSim2}
% \end{figure}

% \begin{figure}[H]
% \centering
% \includegraphics[width=10cm]{plots/plot_sim3_s6_xwoba_check_post.png}
% \caption{Trend in expected wOBA (from Formula~\ref{eqn:xwoba_seq}) over the course of a game from our third simulation study, in which there is pitcher fatigue and a huge 3TTOP. The red dots indicate the ``true'' underlying expected wOBA trajectory, the white dots indicate the posterior means of the expected wOBA values, the thick black error bars denote the 50\% credible intervals, and the thin black error bars denote the 95\% credible intervals. We succesfully recover the ``true'' underlying expected wOBA function.} 
% \label{fig:plotXwobaSim3}
% \end{figure}



% %%%%% REFERENCES
% \clearpage
% \bibliography{../refs}
% \bibliographystyle{plainnat}


